Monitoring the pandemic: A fractional filter for the COVID-19 contact rate

This paper aims to provide reliable estimates for the COVID-19 contact rate of a Susceptible-Infected-Recovered (SIR) model. From observable data on confirmed, recovered, and deceased cases, a noisy measurement for the contact rate can be constructed. To filter out measurement errors and seasonality, a novel unobserved components (UC) model is set up. It specifies the log contact rate as a latent, fractionally integrated process of unknown integration order. The fractional specification reflects key characteristics of aggregate social behavior such as strong persistence and gradual adjustments to new information. A computationally simple modification of the Kalman filter is introduced and is termed the fractional filter. It allows to estimate UC models with richer long-run dynamics, and provides a closed-form expression for the prediction error of UC models. Based on the latter, a conditional-sum-of-squares (CSS) estimator for the model parameters is set up that is shown to be consistent and asymptotically normally distributed. The resulting contact rate estimates for several countries are well in line with the chronology of the pandemic, and allow to identify different contact regimes generated by policy interventions. As the fractional filter is shown to provide precise contact rate estimates at the end of the sample, it bears great potential for monitoring the pandemic in real time.

==> Ch1.tex <==
\section{Introduction}
% HINLEITUNG
What is the long-run growth path of an economy? Do persistent and transitory shocks to economic output correlate? How do private consumption and investment react to periods of economic crises, and which fractions of their reaction can be attributed to permanent and transitory components?
These are key questions in the field of macroeconomic research, and, at least since the seminal work of \cite{Har1985}, unobserved components (UC) models, that decompose a time series into its long-run trend and a transitory cycle, are often the first choice among empirical researchers to assess them.

% ANWENDUNGSÜBERBLICK
\noindent
UC models are widely applied to decompose GDP and to study the cyclical deviations from its long-run trend \citep[][]{MorNelZi2003, MorPig2012}, to estimate the persistent part of industrial production and measure the business cycle \citep[][]{Web2011}, to decompose personal consumption into its long-run and cyclical part \citep[][]{Mor2007}, and to estimate long-run investment \citep[][]{HarTri2003}. By allowing for correlated permanent and transitory shocks, \citet{MorNelZi2003} and \citet{Web2011} draw inference on the (causal) relation between trend and cycle shocks. 

% SPEZIFIKATION DES TRENDS
\noindent
Empirical results differ due to various aspects of model specification. Particularly, the persistence properties of the unobserved components are of crucial importance. Usually, the trend is assumed to be integrated of order one ($I(1)$) as in the aforementioned approaches. In contrast, the double drift model of \cite{Cla1987} and its generalization to correlated unobserved components by \cite{OhZiv2006}, among others, specify a trend that is integrated of order two. This is more in line with earlier, less model-based approaches as the \citet[HP]{HodPre1997} filter \citep[cf.][]{Gom1999, Gom2001}. In yet another approach, building on a specification with structural breaks, \cite{PerWad2009} find the stochastic part of the model to be $I(0)$ for US GDP. Furthermore, \citet{Wad2012} demonstrates that assuming a random walk trend when the true series is $I(0)$ often yields a spurious correlation of -1 or 1 for the estimated innovations. 
Generalizing earlier UC models that assume orthogonality of the different components, \cite{BalWoh2002} and \cite{MorNelZi2003} show identifiability of the unobserved components when correlation among the short- and long-run shocks is allowed. The latter authors find substantial evidence that short- and long-run shocks are highly negatively correlated for US GDP. On the other hand, allowing for correlation among the shocks poses a new problem, as the correlated UC model often produces a volatile trend together with a noisy cycle, thereby contradicting macroeconomic theory \citep[][]{Web2011}.
%In various applications of correlated UC models and the Beveridge-Nelson decomposition, this has led to the unsatisfactory result of volatile trends and noisy cycles \citep[cf.][]{Web2011}.

\noindent
%Misspecification of the integration order is especially damaging in UC models, where the dynamic specification of the components is completely responsible for the decomposition, and can bias both, trend and cycle estimates.

% LONG MEMORY
\noindent
Focusing on key macroeconomic indicators, the assumption of integer integration orders (0, 1, or 2) has been contested for several variables. Most prominently, inflation rates are best modelled by an integration order $d$ between zero and one \citep{HasWol1995, Bai1996, TscWebWe2013, HarTscWeb2019}. For real GDP, \cite{MueWat2017} find that the likelihood is flat around $d=1$, yielding a $90\%$ confidence interval for $d$ that is given by $[0.51, 1.44]$. Inference for $d>1$ is found in \cite{Cha1998} for low frequency transformations of income, consumption, investment, exports, and imports for the UK.


% LONG MEMORY AND UC MODELS
\noindent
If an economic variable violates the assumption of integer integration orders, then the classic UC model misspecifies the long-run dynamics. This poses three major problems. First, since the dynamic specification of the components is responsible for the whole decomposition, misspecifying the long-run dynamics is likely to bias both, trend and cycle estimates. Second, since the consistency argument in \cite{MorNelZi2003} for correlated trend and cycle shocks as well as the consistency proof in \cite{ChaMilPa2009} for data with a common stochastic trend requires that the series under study are $I(1)$, a violation may cause inconsistent parameter estimates. And third, since the current UC framework ignores the presence of $I(d)$ variables, $d \in \mathbb{R}^+$, and specifies its long-run dynamic characteristics typically based on prior unit root tests, model selection uncertainty is not taken into account. 

% CONTRIBUTION
\noindent
We tackle these problems by deriving a fractional trend-cycle decomposition, where the long-run component is allowed to be fractionally integrated ($I(d)$), $d \in \mathbb{R}^+$, whereas the fractional lag operator $L_d = 1-\Delta_+^d$ of \cite{Joh2008}, that is defined in \eqref{diff:op}, enters the lag polynomial of the cyclical component. Since $d$ is defined on a continuous support and enters the likelihood function as an unknown parameter, our model allows for an endogenous estimation of the long-run dynamic characteristics, avoids prior unit root testing and takes into account model selection uncertainty with respect to $d$. 
In UC models fractionally integrated processes allow for richer dynamics of both, trend and cycle components.
The canonical (reduced) form of the fractional trend-cycle model exhibits a fractional ARIMA representation in the fractional lag operator $L_d$. We discuss identification and show that consistency and asymptotic normality carries over from the ARFIMA estimator of \cite{HuaRob2011} and \cite{Nie2015}. Contrary to the correlated UC model, that requires an autoregressive cycle of order $p \geq 2$ to uniquely identify trend and cycle, our model is identified for any $p \geq 0$ whenever $d \neq 1$. 
Finally, we assess the state space representation of the fractional trend-cycle model and propose a computationally efficient modification of the Kalman filter for the estimation of the latent long- and short-run components. 

\noindent
We also contribute to the empirical macroeconomic literature on trend-cycle decompositions by applying our fractional trend-cycle decomposition to US GDP, industrial production, private investment, and personal consumption. Our model nests a wide class of UC models and allows to draw inference on the proper specification of the long-run component for the four series under study. We contrast the trend and cycle estimates from integer-integrated UC models with the results from our fractional decomposition and state differences regarding shape, smoothness, variance and importance of the different components. Especially for industrial production we obtain a decomposition that is in line with economic theory, as the cyclical component captures all NBER recession periods, whereas the correlated UC model clearly fails to produce a plausible cycle. For all time series under study, we estimate a continuous increase of the cyclical components in periods of economic upswing, where the correlated UC model produces a noisy cycle that sharply increases before the economy is hit by a recession.

% OUTLINE
\noindent
The structure of the paper is as follows. Section \ref{Ch:2} details the fractional UC model, relates it to well-established trend-cycle decompositions, derives the reduced form, and discusses identification. Section \ref{sec:ss} derives the state space representation, proposes a computationally efficient modified Kalman filter for the estimation of the latent fractional trend and cycle, and discusses parameter estimation.
In section \ref{sec:app} the model is applied to decompose macroeconomic aggregates. Section \ref{Ch:4} concludes.








==> Ch2.tex <==
\section{A fractional trend-cycle decomposition} \label{Ch:2}
For the trend-cycle decomposition 
\begin{align}\label{eq:t}
	y_t = \tau_t + c_t, \qquad t=1,...,n,
\end{align}
to be suitable to fractionally integrated processes $y_t$, we specify the long-run component $\tau_t$ as a combination of a linear deterministic process and a fractionally integrated series 
\begin{align}\label{eq:tau}
\tau_{t} = \mu_{0} + \mu_{1} t + x_{t}, \qquad \Delta_+^{d}x_{t} = \eta_{t},
\end{align} 
where $\mu_0$ and $\mu_1$ are constants, $d \in \mathbb{R}_+$, and $\eta_{t}$ are the long-run shocks that will be defined in \eqref{eq:shocks} below. The specification \eqref{eq:tau} generalizes the UC literature, where the integration order of $\tau_t$ (and thus also of $y_t$) is typically restricted to $d=1$ \citep[e.g.][]{Har1985, MorNelZi2003}, implying that $x_t$ is a random walk, or to $d=2$ \citep[e.g.][]{Cla1987, OhZiv2006}.
The fractional difference operator $\Delta^{d}$ is defined as
\begin{align}\label{diff:op}
\Delta^{d} &= (1-L)^{d} = \sum_{j = 0}^{\infty}\pi_{j}(d)L^{j},  \qquad
\pi_{j}(d) = 
\begin{cases}
\frac{j-d-1}{j}\pi_{j-1}(d) &  j = 1, 2, ..., \\ 
1										&   j = 0,
\end{cases} 
\end{align}
and a $+$-subscript denotes a truncation of an operator at $t \leq 0$, e.g.\ for an arbitrary process $z_t$, $\Delta_+^d z_t= \sum_{j=0}^{t-1}\pi_j(d) z_{t-j}$ \citep[][def.\ 1]{Joh2008}.
The fractional long-run component $x_t$ adds flexibility to the weighting of past shocks for $d \in \mathbb{R}_+$ and nests the classic integer-integrated specifications for $d \in \mathbb{N}$. The memory parameter $d$ determines the rate at which the autocovariance function of $x_t$ decays, and a higher $d$ implies a slower decay. For $d<1$ $x_t$ is mean-reverting, while $d \in [1, 2)$ yields the aggregate of a mean-reverting process.
Throughout the paper, we adopt the type II definition of fractional integration \citep{MarRob1999} that assumes deterministic starting values for all fractional processes, and, as a consequence, allows for a smooth treatment of the asymptotically stationary ($d < 0.5$) and the nonstationary ($d \geq 0.5$) case. Due to the type II definition of fractional integration the inverse of the fractional difference operator $\Delta_+^{-d} = (1-L)^{-d}_+$ exists for all $d$, so that we can write $x_{t} = \Delta_+^{-d}\eta_t=\sum_{j=0}^{t-1} \pi_j(-d) \eta_{t-j}$ with $\pi_j(-d)$ as given in \eqref{diff:op}. From this, it becomes clear that $\tau_t$ in \eqref{eq:tau} is a type II fractionally integrated process of order $d$ generated by the long-run shocks $\eta_1,...,\eta_t$, where the weights $\pi_j(-d)$ decrease in $j$ if $d<1$, are constant and equal to one if $d=1$, and increase in $j$ if $d>1$.  

Turning to the transitory component, we allow for an AR($p$) process in the fractional lag operator
 \begin{align}\label{eq:c}
 	\phi(L_{d})c_{t}=\varepsilon_{t},
 \end{align}
 where $\phi(L_{d})=1-\phi_{1}L_{d} - ... - \phi_{p} L_{d}^p$, $L_{d} = 1-\Delta^{d}$ is the fractional lag operator \citep[][eq.\ 2]{Joh2008}, and $\varepsilon_{t}$ are the short-run shocks that will be defined in \eqref{eq:shocks} below. For stability of the fractional lag polynomial $\phi(L_{d})$ the condition of \citet[cor.\ 6]{Joh2008} is required to hold. It implies that the roots of $\vert \phi(z) \vert = 0$ lie outside the image $\mathbb{C}_{d}$ of the unit disk under the mapping $z \mapsto 1-(1-z)^{d}$. In fractional models $L_d$ plays the role of the standard lag operator $L_1 = L$, since $(1-L_d) x_t= \Delta^d x_t \sim I(0)$. While for an arbitrary process $z_t$ the standard lag operator $L z_t = (1-(1-L))z_t = z_t - \Delta z_t$ subtracts an $I(-1)$ process from $z_t$, the fractional lag operator $L_d z_t = (1-(1-L_d ))z_t = z_t - \Delta^d z_t$ subtracts an $I(-d)$ process. 
 In addition, $L_d z_t = - \sum_{j=1}^{\infty}\pi_j(d)z_{t-j}$ is a weighted sum of past $z_t$, and hence $L_d$ qualifies as a lag operator. 
 By definition, the filter $\phi(L_{d})$ preserves the integration order of a series since $d > 0$.
 

 Turning to the long- and short-run shocks $\eta_t$, $\varepsilon_t$, we assume that they are white noise with finite third and fourth moments and a non-diagonal covariance matrix $\mQ$, implying
  \begin{align}\label{eq:shocks}
  	 \E 	\begin{pmatrix}
  			\eta_{t} \\ \varepsilon_{t} 
  	 	\end{pmatrix} =0, \quad 
  		 \Var	\begin{pmatrix}
  		 	\eta_{t} \\ \varepsilon_{t} 
  		 \end{pmatrix}=\mQ = \begin{bmatrix}
  		 	\sigma_\eta^2 & \sigma_{\eta \varepsilon} \\
  		 	\sigma_{\eta \varepsilon} & \sigma_\varepsilon^2
  	 \end{bmatrix}, \quad 
   	\Cov \left[\begin{pmatrix}
   		\eta_{t} \\ \varepsilon_{t} 
   	\end{pmatrix}, \begin{pmatrix}
   	\eta_{t-s} \\ \varepsilon_{t-s} 
   \end{pmatrix}  \right] = 0_{2,2} \  \forall s\neq0.
\end{align}
This is somewhat more general than the bulk of the literature on UC models that requires the shocks to be Gaussian white noise \citep[e.g.][]{MorNelZi2003, PerWad2009}. The white noise assumption is required for the disturbances of the reduced form to aggregate to a moving average process via Grangers lemma \citep{GraMor1976}, as will become clear in \eqref{eq:fBN} and \eqref{eq:farima} below. Note that the model allows for contemporaneous correlation between trend and cycle innovations, $\rho = \Corr(\eta_t, \varepsilon_t) \neq 0$.


%All unknown model parameters are collected in a vector $\vtheta = (d, \phi_1,...,\phi_p, \sigma_\eta^2, \sigma_{\eta \varepsilon}, \sigma_\varepsilon^2)' \in \mTheta$, and we denote the data-generating parameter vector $\vtheta_0 \in \mTheta$. $\mTheta$ is the parameter space and is convex and compact.

 
 Our UC model in \eqref{eq:t}, \eqref{eq:tau}, \eqref{eq:c}, and \eqref{eq:shocks} is very general in terms of its long-run dynamic characteristics, as it nests the well-known framework of \cite{Har1985} for $d=1$, $\sigma_{\eta \varepsilon}=0$, where the long-run component is a random walk with drift, and $c_{t}$ is an autoregressive process of finite order. Correlated shocks as in \cite{BalWoh2002}, \cite{MorNelZi2003}, and \cite{Web2011} are explicitly allowed. For $d=2$, one obtains the double-drift model of \cite{Cla1987}, and a fractional plus noise decomposition as proposed in \cite{Har2002} for stochastic volatility modelling is obtained by setting $d \in \mathbb{R}_+$, $p=0$. As will become clear in section \ref{sec:app}, the model can easily be enriched to encompass trend breaks as in \cite{PerWad2009}.

% REDUCED FORM
One interesting property of the fractional UC model is that it can be interpreted as a generalization of the decomposition of \cite{BevNel1981} to the fractional domain. To see this, plug \eqref{eq:tau} and \eqref{eq:c} into \eqref{eq:t} and take fractional differences. Then 
\begin{align}\label{eq:fBN1}
	\Delta^{d}_+(y_{t} - \mu_{0}-\mu_{1} t )=  \eta_{t} + \Delta_+^d\phi(L_{d})^{-1} \varepsilon_{t},
\end{align}
 where  $\phi(L_{d})^{-1}$ exists since $\phi(L_d)$ is stable. For an arbitrary $z_t$, define $\Delta_{-}^{d} z_t = \Delta^d z_t - \Delta_{+}^d z_t$ as the fraction of the polynomial $\Delta^d$ that is truncated away, and note that for an $I(0)$ process $z_t$, $\Delta_{-}^{d} z_t = \sum_{j=t}^\infty \pi_j(d)z_{t-j} = o_p(1)$ since $\pi_j(d) = O(j^{-d-1})$ \citep[][eq.\ 5.25]{Has2018}. We denote $r(t, d, \phi) = - \Delta_{-}^d\phi(L_{d})^{-1} \varepsilon_{t} = o_p(1)$ and write $ \Delta_+^d\phi(L_{d})^{-1} \varepsilon_{t} = \Delta^d\phi(L_{d})^{-1} \varepsilon_{t} + r(t, d, \phi) = (1-L_d)\phi(L_{d})^{-1} \varepsilon_{t} +  r(t, d, \phi) = \theta^\varepsilon(L_d)\varepsilon_t +r(t, d, \phi)$, with $\theta^\varepsilon(L_d) = (1-L_d)\phi(L_{d})^{-1}$ as an infinite MA polynomial in the fractional lag operator which follows since $\phi(L_d)$ is invertible. Plugging this result into \eqref{eq:fBN1} then yields an ARFIMA model in the fractional lag operator $L_d$
\begin{align}
	\Delta^{d}_+(y_{t} - \mu_{0}-\mu_{1} t )&=  \eta_{t} + \theta^\varepsilon(L_{d}) \varepsilon_{t} + r(t, d, \phi)= \theta^u(L_{d})u_{t} + r(t, d, \phi), \label{eq:fBN}
\end{align} 
where $u_t$ is white noise with $\Var(u_t) = \sigma_u^2 = \sigma_\eta^2 + \sigma_\varepsilon^2 + 2\sigma_{\eta \varepsilon}$, and $\theta^{u}(L_d) = 1 + \sum_{j=1}^\infty \theta_j^u L_d^j$. The last equality in \eqref{eq:fBN} follows from the aggregation properties of MA processes in the fractional lag operator with white noise innovations, as shown in appendix \ref{App:MA_agg} where also a recursive formula for the $\theta_j^u$ is derived. For the particular case in \eqref{eq:fBN}, where a white noise process is added to an MA process in the fractional lag operator, it follows that $\theta^u_j = \theta^\varepsilon_j (\sigma_\varepsilon / \sigma_u)$, $j=1,2,...$. 
%The last equality follows from $\phi(L_d)$ being a stably polynomial for any $d$ by construction, so that its inverse $\phi(L_d)^{-1}$ is a stably MA polynomial of order infinity that is truncated by the fractional difference operator $\Delta_+^d$. Thus, $\Delta_+^d \phi(L_d)^{-1}\varepsilon_t = \theta^\varepsilon(L) \varepsilon_t = \sum_{j=0}^{t-1} \theta^\varepsilon_j \varepsilon_{t-j}$ yields an MA($n-1$) process that is $I(-d)$ and, thus, stationary. Since $\eta_t \sim I(0)$, it dominates the integration order of $\theta^\varepsilon(L)\varepsilon_t$, so that their sum is $I(0)$. Finally, since the sum of two contemporaneously correlated MA processes with white noise shocks is a MA process whose order equals the higher lag order of the two underlying MA processes, $\theta_+^u(L_{d})u_{t} = \sum_{j=0}^{t-1} \theta^u_j u_{t-j} \sim I(0)$ with $u_t \sim WN(0, \sigma_u^2)$ and finite third and fourth moments, $\sigma_u^2 = \sigma_\eta^2 + \sigma_\varepsilon^2 + 2 \sigma_{\eta \varepsilon}$, and the coefficients $\theta_0^u = 1$, $\theta_j^u =( \sigma_\varepsilon / \sigma_u) \theta^\varepsilon_j $ for all $j\geq 1$ follow from matching the autocovariance functions of \eqref{eq:fBN}. 



From \eqref{eq:fBN} the fractional Beveridge-Nelson decomposition follows directly
\begin{align*}
	\Delta_+^d (y_{t} - \mu_{0} - \mu_{1}t) &=  \vtheta^u(L_d) u_{t} +r(t, d, \phi)= \theta^u(1) u_{t} - (1-L_{d}) \sum_{k=0}^{\infty} L_{d}^k u_{t} \sum_{j=k+1}^{\infty}\theta_{j}^u +r(t, d, \phi),
\end{align*} 
so that multiplication with $\Delta_+^{-d}$ yields the long- and short-run components 
\begin{align}\label{eq:BN}
	x^{BN}_{t} = \Delta^{-d}_+ \vtheta^u(1) u_{t} = x_t, \qquad c_{t}^{BN} = - \sum_{k=0}^{\infty} L_{d}^k u_{t} \sum_{j=k+1}^{\infty}\theta_{j}^u =c_t,
\end{align}
where we use $\Delta_+^{-d} r(t, d, \phi) = 0$, since $r(t, d, \phi)$ only depends on $\varepsilon_j$, $j\leq 0$, and thus all coefficients in $\Delta_+^{-d} $ attached to $r(t, d, \phi)$ are zero.
While it was shown by \cite{MorNelZi2003} that the UC model in \eqref{eq:t}, \eqref{eq:tau}, and \eqref{eq:c} has a Beveridge-Nelson decomposition for $d=1$, this carries over directly to the fractional case. $x_t^{BN}$ and $c_t^{BN}$ are identical to the unobserved components in \eqref{eq:tau} and \eqref{eq:c} for any $d$, which follows immediately from plugging $L_d = 1$ in \eqref{eq:fBN} and multiplying with $\Delta_+^{-d}$, since $\theta^\varepsilon(L_d) = (1-L_d)\phi(L_d)^{-1}$ is zero for $L_d=1$ and $\Delta_+^{-d}r(t, d, \phi)=0$. Consequently, the fractional trend-cycle decomposition generalizes the $I(1)$ Beveridge-Nelson decomposition to the class of ARFIMA models in the fractional lag operator. 



 

==> macros.tex <==
% !TeX encoding = UTF-8
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% symbols C,N,Q,R,Z for sets
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\C}{\mathbb{C}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\D}{\mathbb{D}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% timestamps
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\monthword}[1]{\ifcase#1\or Jan\or Feb\or M\"ar\or Apr\or Mai\or Jun\or Jul\or Aug\or Sep\or Okt\or Nov\or Dez\fi}
\newcommand{\leadingzero}[1]{\ifnum #1<10 0\the#1\else\the#1\fi}             %%fügt bei 1 bis 9 eine führende Null an

\newcommand{\todayI}{\the\year"~\leadingzero{\month}"~\leadingzero{\day}}    	%%YYYY-MM-DD
\newcommand{\todayII}{\the\year\leadingzero{\month}\leadingzero{\day}}       	%%YYYYMMDD
\newcommand{\todayIII}{\leadingzero{\day}/\leadingzero{\month}/\the\year}    	%%DD/MM/YYYY
\newcommand{\todayIV}{\leadingzero{\day}.\leadingzero{\month}.\the\year}     	%%DD.MM.YYYY
\newcommand{\todayV}{\the\day.\the\month.\the\year}                          	%%D.M.YYYY
\newcommand{\todayVI}{\the\day.~\monthword{\the\month}. \the\year}           	%%D. MMM. YYYY
\newcommand{\todayVII}{\leadingzero{\day}.~\monthword{\the\month}. \the\year}	%%DD. MMM. YYYY
\newcommand{\todayVIII}{\monthword{\the\month}. \the\year}										%%DD. MMM. YYYY

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% calligraphic capital letters
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\calA}{\mathcal{A}}
\newcommand{\calB}{\mathcal{B}}
\newcommand{\calC}{\mathcal{C}}
\newcommand{\calD}{\mathcal{D}}
\newcommand{\calE}{\mathcal{E}}
\newcommand{\calF}{\mathcal{F}}
\newcommand{\calG}{\mathcal{G}}
\newcommand{\calH}{\mathcal{H}}
\newcommand{\calI}{\mathcal{I}}
\newcommand{\calJ}{\mathcal{J}}
\newcommand{\calK}{\mathcal{K}}
\newcommand{\calL}{\mathcal{L}}
\newcommand{\calM}{\mathcal{M}}
\newcommand{\calN}{\mathcal{N}}
\newcommand{\calO}{\mathcal{O}}
\newcommand{\calP}{\mathcal{P}}
\newcommand{\calQ}{\mathcal{Q}}
\newcommand{\calR}{\mathcal{R}}
\newcommand{\calS}{\mathcal{S}}
\newcommand{\calT}{\mathcal{T}}
\newcommand{\calU}{\mathcal{U}}
\newcommand{\calV}{\mathcal{V}}
\newcommand{\calW}{\mathcal{W}}
\newcommand{\calX}{\mathcal{X}}
\newcommand{\calY}{\mathcal{Y}}
\newcommand{\calZ}{\mathcal{Z}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% bold lowercase and capital letters for vectors (v) and matrices (m)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\newcommand{\bm}[1]{{\boldmath #1}}

\newcommand{\mA}{\bm A}
\newcommand{\va}{\bm a}
\newcommand{\mB}{\bm B}
\newcommand{\vb}{\bm b}
\newcommand{\mC}{\bm C}
\newcommand{\vc}{\bm c}
\newcommand{\mD}{\bm D}
\newcommand{\vd}{\bm d}
\newcommand{\mE}{\bm E}
\newcommand{\ve}{\bm e}
\newcommand{\mF}{\bm F}
\newcommand{\vf}{\bm f}
\newcommand{\mG}{\bm G}
\newcommand{\vg}{\bm g}
\newcommand{\mH}{\bm H}
\newcommand{\vh}{\bm h}
\newcommand{\mI}{\bm I}
\newcommand{\vi}{\bm i}
\newcommand{\mJ}{\bm J}
\newcommand{\vj}{\bm j}
\newcommand{\mK}{\bm K}
\newcommand{\vk}{\bm k}
\newcommand{\mL}{\bm L}
\newcommand{\vl}{\bm l}
\newcommand{\mM}{\bm M}
\newcommand{\vm}{\bm m}
\newcommand{\mN}{\bm N}
\newcommand{\vn}{\bm n}
\newcommand{\mO}{\bm O}
\newcommand{\vo}{\bm o}
\newcommand{\mP}{\bm P}
\newcommand{\vp}{\bm p}
\newcommand{\mQ}{\bm Q}
\newcommand{\vq}{\bm q}
\newcommand{\mR}{\bm R}
\newcommand{\vr}{\bm r}
\newcommand{\mS}{\bm S}
\newcommand{\vs}{\bm s}
\newcommand{\mT}{\bm T}
\newcommand{\vt}{\bm t}
\newcommand{\mU}{\bm U}
\newcommand{\vu}{\bm u}
\newcommand{\mV}{\bm V}
\newcommand{\vv}{\bm v}
\newcommand{\mW}{\bm W}
\newcommand{\vw}{\bm w}
\newcommand{\mX}{\bm X}
\newcommand{\vx}{\bm x}
\newcommand{\mY}{\bm Y}
\newcommand{\vy}{\bm y}
\newcommand{\mZ}{\bm Z}
\newcommand{\vz}{\bm z}

\newcommand{\vnull}{\bm 0}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% beta und gamma as estimators
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\muh}{\hat{\mu}}
\newcommand{\mut}{\tilde{\mu}}
\newcommand{\uh}{\hat{\vu}}
\newcommand{\yh}{\hat{\vy}}

\newcommand{\hbeta}{\hat{\beta}}
\newcommand{\tbeta}{\tilde{\beta}}
\newcommand{\bbeta}{\boldsymbol{\beta}}
\newcommand{\hbbeta}{\hat{\bbeta}}

\newcommand{\hgamma}{\hat{\gamma}}
\newcommand{\tgamma}{\tilde{\gamma}}
\newcommand{\bgamma}{\mathbf{\gamma}}
\newcommand{\hbgamma}{\hat{\bgamma}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% bold Greek lowercase letters for vectors (v)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\valpha}{\bm \alpha}
\newcommand{\vbeta}{\bm \beta}
\newcommand{\hvbeta}{\hat{\vbeta}}
\newcommand{\tvbeta}{\tilde{\vbeta}}
\newcommand{\vgamma}{\bm \gamma}
\newcommand{\vdelta}{\bm \delta}
\newcommand{\vepsi}{\bm \epsi}
\newcommand{\vvarepsilon}{\bm \varepsilon}
\newcommand{\vzeta}{\bm \zeta}
\newcommand{\veta}{\bm \eta}
\newcommand{\vtheta}{\bm \theta}
\newcommand{\viota}{\bm \iota}
\newcommand{\vkappa}{\bm \kappa}
\newcommand{\vlambda}{\bm \lambda}
\newcommand{\vmu}{\bm \mu}
\newcommand{\vnu}{\bm \nu}
\newcommand{\vxi}{\bm \xi}
\newcommand{\vpi}{\bm \pi}
\newcommand{\vrho}{\bm \rho}
\newcommand{\vsigma}{\bm \sigma}
\newcommand{\vtau}{\bm \tau}
\newcommand{\vupsilon}{\bm \upsilon}
\newcommand{\vphi}{\bm \phi}
\newcommand{\vchi}{\bm \chi}
\newcommand{\vpsi}{\bm \psi}
\newcommand{\vomega}{\bm \omega}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% bold Greek capital letters for matrices (m)
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\mGamma}{\bm \varGamma}
\newcommand{\mDelta}{\bm \varDelta}
\newcommand{\mTheta}{\bm \varTheta}
\newcommand{\mLambda}{\bm \varLambda}
\newcommand{\mXi}{\bm \varXi}
\newcommand{\mPi}{\bm \varPi}
\newcommand{\mSigma}{\bm \varSigma}
\newcommand{\mUpsilon}{\bm \varUpsilon}
\newcommand{\mPhi}{\bm \varPhi}
\newcommand{\mPsi}{\bm \varPsi}
\newcommand{\mOmega}{\bm \varOmega}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% roman letters in mathematics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\rb}{\ensuremath{\mathrm{b}}}
\newcommand{\rB}{\ensuremath{\mathrm{B}}}
\newcommand{\rC}{\ensuremath{\mathrm{C}}}
\newcommand{\rD}{\ensuremath{\mathrm{D}}}
\newcommand{\rf}{\ensuremath{\mathrm{f}}}
\newcommand{\rF}{\ensuremath{\mathrm{F}}}
\newcommand{\rH}{\ensuremath{\mathrm{H}}}
\newcommand{\rL}{\ensuremath{\mathrm{L}}}
\newcommand{\rN}{\ensuremath{\mathrm{N}}}
\newcommand{\rt}{\ensuremath{\mathrm{t}}}
\newcommand{\rU}{\ensuremath{\mathrm{U}}}
\newcommand{\rGam}{\ensuremath{\mathrm{Gam}}}
\newcommand{\rBeta}{\ensuremath{\mathrm{Beta}}}
%
\newcommand{\Bin}{\ensuremath{\mathrm{Bin}}}
\newcommand{\eu}{\ensuremath{\mathrm{e}}}
\newcommand{\iu}{\ensuremath{\mathrm{i}}}
\newcommand{\LN}{\ensuremath{\mathrm{LN}}}
\newcommand{\IN}{\ensuremath{\mathrm{IN}}}

\newcommand{\Poi}{\ensuremath{\mathrm{Poi}}}
%
\newcommand{\ped}[1]{\ensuremath{_\mathrm{#1}}} %pedex
\newcommand{\ap}[1]{\ensuremath{^\mathrm{#1}}} %apex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% fractal letters in mathematics
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\frakA}{\mathfrak{A}}
\newcommand{\frakB}{\mathfrak{B}}
\newcommand{\frakF}{\mathfrak{F}}
\newcommand{\frakO}{\mathfrak{O}}
\newcommand{\frakZ}{\mathfrak{Z}}
\newcommand{\frakC}{\mathfrak{C}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% letters for (partial) differentiation
%\newcommand{\rd}{\ensuremath{\mathrm{d}}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\makeatletter
\newcommand{\rd}{\@ifnextchar^{\DIfF}{\DIfF^{}}}
\def\DIfF^#1{%
   \mathop{\mathrm{\mathstrut d}}%
   \nolimits^{#1}\gobblespace}
\def\gobblespace{\futurelet\diffarg\opspace}
\def\opspace{%
   \let\DiffSpace\!%
   \ifx\diffarg(%
   \let\DiffSpace\relax
   \else
   \ifx\diffarg[%
   \let\DiffSpace\relax
   \else
   \ifx\diffarg\{%
   \let\DiffSpace\relax
   \fi\fi\fi\DiffSpace}
\newcommand{\deriv}[3][]{\frac{\rd^{#1}#2}{\rd #3^{#1}}}
\newcommand{\pderiv}[3][]{\frac{\partial^{#1}#2}{\partial #3^{#1}}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% operatornames
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\bias}{\operatorname{bias}}
\newcommand{\col}{\operatorname{col}}
\newcommand{\dg}{\operatorname{dg}}
\newcommand{\diag}{\operatorname{diag}}
\newcommand{\etr}{\operatorname{etr}}
\newcommand{\kur}{\operatorname{kur}}
\newcommand{\median}{\operatorname{med}}
\newcommand{\MSE}{\operatorname{MSE}}
\newcommand{\rk}{\operatorname{rk}}
\newcommand{\sgn}{\operatorname{sgn}}
\newcommand{\vech}{\operatorname{vech}}
\newcommand{\id}{\operatorname{id}}
\newcommand{\tr}{\operatorname{tr}}
\newcommand{\Mor}{\operatorname{Mor}}
\newcommand{\Abb}{\operatorname{Abb}}
\newcommand{\Lin}{\operatorname{Lin}}
\newcommand{\Real}{\operatorname{Re}}
\newcommand{\Image}{\operatorname{Im}}
\newcommand{\End}{\operatorname{End}}
\newcommand{\ggT}{\operatorname{ggT}}
\newcommand{\Ker}{\operatorname{Ker}}
\newcommand{\coker}{\operatorname{coker}}
\newcommand{\Hom}{\operatorname{Hom}}
\newcommand{\Ann}{\operatorname{Ann}}
\newcommand{\Frac}{\operatorname{Frac}}
\newcommand{\Spec}{{\operatorname{Spec}\,}}
\newcommand{\Proj}{{\operatorname{Proj}\,}}
\newcommand{\codim}{\operatorname{codim}}
\newcommand{\kon}{\operatorname{kon}}
\newcommand{\res}{\operatorname{res}}
\newcommand{\kor}{\operatorname{kor}}
\newcommand{\ad}{\operatorname{ad}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% other definitions
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\adistr}{\stackrel{a}{\distr}}
\newcommand{\diff}{\Delta}
\newcommand{\fdiff}{\diff_{\rf}}
\newcommand{\bdiff}{\diff_{\rb}}
\newcommand{\eps}{\epsilon}
\newcommand{\epsi}{\varepsilon}
%
\newcommand{\longto}{\longrightarrow}
\newcommand{\pto}{\stackrel{p}{\longrightarrow}}
\newcommand{\dto}{\stackrel{d}{\longrightarrow}}
\newcommand{\wto}{\stackrel{w}{\longrightarrow}}
%
\newcommand{\Infmat}{\bm\calI}
\newcommand{\Hesmat}{\bm\calH}
\newcommand{\bcdot}{\raisebox{1pt}{\textbf{\large .}}}
%
\newcommand{\vones}{\bm\imath}
\newcommand{\vzeros}{\boldsymbol{0}}
\newcommand{\mZeros}{\mathbf{O}}
%
% additional commands
\newcommand{\interior}[1]{\overset{\circ}{#1}}
\newcommand{\mzeros}{\mZeros}
\newcommand{\mply}{\cdot}
\newcommand{\widebar}{\overline}
\newcommand{\bin}{\Bin}
\newcommand{\Po}{\Poi}
\newcommand{\e}{\eu}% exponential e
\newcommand{\E}[1]{\operatorname{E}[#1]}
\newcommand{\Var}[1]{\operatorname{Var}\left(#1\right)}
\newcommand{\Cov}[1]{\operatorname{Cov}\left(#1\right)}
\newcommand{\Corr}[1]{\operatorname{Corr}\left(#1\right)}
\newcommand{\prob}[1]{\P\left(#1\right)}
\newcommand{\MAX}[1]{\max\left\{#1\right\}}
\newcommand{\MIN}[1]{\min\left\{#1\right\}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Own abbreviations and commands:
% Aufgaben als sections
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\aufgabe}[1]{\section{#1}
\vspace*{-0.4 cm}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Pfeile
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\ra}{\longrightarrow}
\newcommand{\Ra}{\Longrightarrow}
\newcommand{\la}{\longleftarrow}
\newcommand{\La}{\Longleftarrow}
\newcommand{\LR}{\Longleftrightarrow}
\newcommand{\lr}{\longleftrightarrow}
\newcommand{\PRa}{\overset{P}{\longrightarrow}}
\newcommand{\PLa}{\overset{P}{\longleftarrow}}
\newcommand{\DRa}{\overset{d}{\longrightarrow}}
\newcommand{\DLa}{\overset{d}{\longleftarrow}}
\newcommand{\ARa}{\overset{a.s.}{\longrightarrow}}
\newcommand{\ALa}{\overset{a.s.}{\longleftarrow}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Limiten, Summen andere Mengenoperatoren
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand{\lim}[1]{\underset{#1}{\operatorname{lim}} \;}
\newcommand{\plim}[1]{\underset{#1}{\operatorname{plim}} \;}
\renewcommand{\sup}[1]{\underset{#1}{sup} \;}
\renewcommand{\inf}[1]{\underset{#1}{inf} \;}
\renewcommand{\max}[1]{\underset{#1}{\operatorname{max}} \;}
\renewcommand{\min}[1]{\underset{#1}{min} \;}
\newcommand{\limni}{\lim{n \to \infty} \;}
\newcommand{\limxi}{\lim{x \to \infty} \;}
\newcommand{\limzi}{\lim{z \to \infty} \;}
\newcommand{\plimni}{\plim{n \to \infty} \;}
\newcommand{\plimti}{\plim{t \to \infty} \;}
\newcommand{\tsum}{\sum_{t=1}^T \;}
\newcommand{\nsum}{\sum_{t=1}^T \;}
\newcommand{\bb }[1]{\bold  {#1}}
\newcommand{\bs }[1]{\boldsymbol {#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Umgebungen
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% a) b) c) Zähler in jeder Section durchlaufend

